Question Answering as Global Reasoning over Semantic Abstractions

We propose a novel method for exploiting the semantic structure of text to answer multiple-choice questions. The approach is especially suitable for domains that require reasoning over a diverse set of linguistic constructs but have limited training data. To address these challenges, we present the first system, to the best of our knowledge, that reasons over a wide range of semantic abstractions of the text, which are derived using off-the-shelf, general-purpose, pre-trained natural language modules such as semantic role labelers, coreference resolvers, and dependency parsers. Representing multiple abstractions as a family of graphs, we translate question answering (QA) into a search for an optimal subgraph that satisfies certain global and local properties. This formulation generalizes several prior structured QA systems. Our system, SEMANTICILP, demonstrates strong performance on two domains simultaneously. In particular, on a collection of challenging science QA datasets, it outperforms various state-of-the-art approaches, including neural models, broad coverage information retrieval, and specialized techniques using structured knowledge bases, by 2%-6%.

==> intro-no-longer-used.tex <==

\section{Introduction}

Question answering (QA) is a fundamental challenge in AI, particularly in natural language processing (NLP) and reasoning. We consider the multiple-choice setting where $Q$ is a question, $A$ is a set of answer candidates, and the knowledge required for answering $Q$ is available in the form of raw text $P$. This setting applies naturally to reading comprehension questions, as well as to open format multiple-choice questions for which information retrieval (IR) techniques are able to obtain relevant text from a corpus.

Several state-of-the-art QA systems excel at locating the correct answer in $P$ based on proximity to question words, the distributional semantics of the text, answer type, etc \cite{aristo2016:combining},
% \daniel{cite something here?}. Even the best solvers
however, often struggle with questions that require some form of reasoning or appeal to a more subtle 
%linguistic 
understanding of the supporting text or the question. We demonstrate that we can use existing NLP modules, such as semantic role labeling (SRL) systems with respect to multiple predicate types (verbs, prepositions, nominals, etc.),
%\daniel{predicates $\rightarrow$ predicate types}, 
%\dan{Note that most people think of SRL only wrt verbs; thus the change.}
to derive multiple semantic views of the text and perform reasoning over these views to answer a variety of questions.

% {\color{blue}
As an example, consider the following snippet of sports news text and an associated question:
\begin{framed}
%\vspace{-1.5ex}
\noindent\footnotesize\emph{\noindent$P$: Teams are under pressure after PSG purchased Neymar this season. \textbf{Chelsea purchased Morata}. The Spaniard looked like he was set for a move to Old Trafford for the majority of the summer only for Manchester United to sign Romelu Lukaku instead, paving the way for Morata to finally move to Chelsea for an initial \pounds 56m.
%The 24-year-old is in line to make his full Chelsea debut on Sunday against Tottenham at Wembley on Sunday having come off the bench in the season’s curtain raiser against Burnley last weekend.   
%He made a positive start to life in west London with a goal and an assist despite that defeat and Conte insisted that given today market – where Liverpool are rejecting £110m+ offers for Philippe Coutinho – Morata is a bargain signing for the Blues. After signing Morata, Conte spoke publically of how Spurs striker Kane would have been is ideal signing but he tried to clarify those comments by insisting Morata can have a similar impact to the Englishman. 
% }
% \end{framed}
% And consider the following question: 
% \begin{framed}
% \small
\\
\noindent
$Q$: Who did Chelsea purchase this season?  \\ 
$A$: \{\checkmark Alvaro Morata, Neymar, Romelu Lukaku \}%  \;  (D) Manchester United
}
%\vspace{-1.5ex}
\end{framed}

Given the bold-faced text $P'$ in $P$, simple word-matching suffices to correctly answer $Q$. However, $P'$ could have stated the same information in many different ways. As paraphrases become more complex, they begin to involve more linguistic constructs such as coreference, punctuation, prepositions, and nominals. This makes understanding the text, and thus the QA task, more challenging.

For instead, $P'$ could instead say \emph{Morata is the recent \textbf{acquisition} by Chelsea}. This simple looking transformation can be surprisingly confusing for highly successful systems such as \bidaf~\cite{seo2016bidirectional}, which produces the partially correct phrase \emph{``Neymar this season.\ Morata''}. On the other hand, one can still answer the question confidently by abstracting relevant parts of $Q$ and $P$, and connecting them appropriately. Specifically, a verb SRL frame for $Q$ would indicate that we seek the object of the verb \emph{purchase}, a nominal SRL frame for $P'$ would capture that the \emph{acquisition} was of Morata and was done by Chelsea, and textual similarity would align \emph{purchase} with \emph{acquisition}.

\begin{figure}[ht]
    \centering
    % \begin{framed}
    % \includegraphics[trim=-0.00cm 3.7cm 0cm -0.00cm, scale=0.53]{figures/Chelseaishopingtohaveagreatstartthisseason3}
    % \end{framed}
    % \includegraphics[trim=-0.00cm 2.5cm 2.5cm -0.00cm, scale=0.55]{figures/cropped_morata-simplfied-cropped.pdf}
    \includegraphics[trim=-0.00cm 0cm 0cm -0.00cm, scale=0.55]{figures/cropped_morata-simplfied-cropped.pdf}
    \caption{Depiction of \textilp\ reasoning for the example paragraph given in the text.
    Semantic abstractions of the question, answers, knowledge snippet are shown in different colored boxes (blue, green, and yellow, resp.). Red nodes and edges are the elements that are aligned (used) for supporting the correct answer. There are many other unaligned (unused) annotations associated with each piece of text that are omitted for clarity. 
    }
    \label{fig:morata-visualization}
\end{figure}

Similarly, suppose $P'$ instead said \emph{Morata\textbf{,} the recent acquisition \textbf{by} Chelsea\textbf{,} will start for the team tomorrow.} \bidaf\ now incorrectly chooses Neymar as the answer, presumably due to its proximity to the words \emph{purchased} and \emph{this season}. However, with the right abstractions, one could still arrive at the correct answer as depicted in Figure~\ref{fig:morata-visualization} for our proposed system, \textilp. This reasoning uses comma SRL to realize that the Morata is referring to the \emph{acquisition}, and a preposition SRL frame to capture that the acquisition was done \emph{by} Chelsea.

One can continue to make $P'$ more complex. For example, $P'$ could introduce the need for coreference resolution by phrasing the information as: \emph{\textbf{Chelsea} is hoping to have a great start this season by actively hunting for new players in the transfer period. Morata, the recent acquisition by the team, will start for \textbf{the team} tomorrow.} Nevertheless, with appropriate semantic abstractions of the text, the underlying reasoning remains relatively simple. 

% such as:
% \begin{framed}
% \vspace{-3ex}
% \footnotesize
%     \emph{ 
%     \begin{enumerate}[leftmargin=0.3cm]
%         \item Chelsea acquired Alvaro Morata.  
%         \item Real Madrid sold Alvaro Morata to Chelsea. 
%         % \item Alvaro Morata's recent acquisition by Chelsea has given extra hope for its fans.  
%         \item Chelsea broke its previous record by purchasing Morata from Real Madrid. \ashish{SQuAD: Morata from Real Madrid}
%         \item Morata hinted at his purchase. Later that day Chelsea announced the purchase.  
%         \item Recent purchase for Chelsea, Alvaro Morata, will start for Chelsea tomorrow.
%         \item Chelsea is hoping to have a great start this season by actively hunting for new players in the transfer period. Morata, the recent acquisition by the team, will start for the team tomorrow.
%     \end{enumerate}
%     }
% \vspace{-2ex}
% \end{framed}

% The first paraphrasing of $P'$ relies on synonymy between \emph{purchased} and \emph{acquired}, a gap easily bridged using resources such as WordNet~\cite{miller1995wordnet} or low-dimensional word embeddings~\cite{mikolov2013distributed}. The second requires understanding that \emph{X purchased Y} is the same as \emph{Y was sold to X}, which methods using contextual verb embeddings, such as LSTM based neural models~\cite{?}, may be able to address. \daniel{instead of this I would say, ``The second requires understanding that \emph{X purchased Y} is the same as \emph{Y was sold to X}, which resources like PropBank~\cite{kingsbury2002treebank} would help to answer."} \ashish{Agreed with the explanation, although, especially since even we don't use PropBank and get it right, I would instead change the rephrasing of $T'$ so that it requires more than just soft word distance but a state-of-the-art system like BiDAF \emph{can} get it correct. Then say what it cannot get.}
% \dan{Are you sure that LSTM based  systems get it for the right reason? Or only because it's the only NE option? Can you try to add deceiving entities?}
% \ashish{Not sure about LSTM. The text does have all other answer options (also NEs) mentioned in the second sentence of the paragraph.}
% \dan{Maybe it's sufficient to say: "requires understanding that \emph{X purchased Y} is the same as \emph{Y was sold to X}"; [or add also] a lexico-structural pattern that can be learned from a large QA collection only for the most common lexical items.}
% \ashish{I like the fancy last sentence, in part because it yields that existing systems \emph{can} do this, at least for common terms.}
% % side note: Propbank indeed helps us answer this. If you go to the "sell" frame, it labels subject as "buyer": https://github.com/propbank/propbank-frames/blob/master/frames/sell.xml#L21
% % }


Given sufficiently large QA training data, one could conceivably perform end-to-end training (e.g., using a deep learning method) to address these linguistic challenges. However, existing large scale QA datasets such as SQuAD~\cite{Rajpurkar2016SQuAD10} often either have a limited linguistic richness or do not necessarily need reasoning to arrive at the answer~\cite{Jia2017AdversarialEF}. 
% \ashish{update citation to point to EMNLP (I think)} 
%\danchange{
Consequently, the resulting models do not transfer easily to other domains.
%}
%\dan{is there a reference to cite here?; can we give the performance of a good Squad system on Aristo?} \ashish{added SQuAD-trained BiDAF performance on Aristo. Helpful or risky claim?}. 
For instance, the above mentioned BiDAF model trained on the SQuAD dataset performs substantially worse than a simple IR approach on our datasets. On the other hand, many of the QA collections in domains that require some form of reasoning, such as the science questions we use, are small  
%, suffer from the issue of \emph{data sparsity}. Their small size 
(100s to 1000s of questions). This brings into question the viability of the aforementioned paradigm that attempts 
%makes it difficult, if not impossible, 
to learn everything from only the QA training data. %One is thus limited to fine tuning parameters of a system pre-trained on a different, larger dataset.
% \dan{rephrased the previous paragraph a bit; please check}\ashish{nice!}

Towards the goal of effective structured reasoning in the presence of data sparsity, we propose to use a rich set of general-purpose, pre-trained NLP tools to create various \emph{semantic abstractions} of the raw text\footnote{This applies to all three inputs of the system: $Q$, $A$, and $P$.} in a domain independent fashion, as illustrated for an example in Figure~\ref{fig:morata-visualization}.
%
%For instance, \ashish{TO-DO: connect back to the illustrative examples above}
% {\color{blue}
% in the 3rd rephrasing above, a semantic role labeling (SRL) system for verbs may identify \emph{Chelsea} as the \emph{purchaser}, despite the presence of several other words in between the verb and its subject. In the 4th rephrasing, a coreference system may reveal that the two mentions of \emph{purchase} refer to the same real-life event. An SRL system for the semantics of commas may similarly identify, in the 5th rephrasing, \emph{Alvaro Morata} as being interchangeable with \emph{recent purchase}. Finally, as the last rephrasing illustrates, one may need to resort to \emph{multiple semantic abstractions} simultaneously.
% }
%
We represent these semantic abstractions as \emph{families of graphs}, where the family (e.g., trees, clusters, labeled predicate-argument graphs, etc.) is chosen to match the nature of the abstraction (e.g., parse tree, coreference sets, SRL frames, etc., respectively). The collection of semantic graphs is then augmented with inter- and intra-graph edges capturing lexical similarity (e.g., word-overlap score or word2vec distance).
%Figure~\ref{fig:morata-visualization} illustrates what such a graph looks like. \ashish{TO-DO: change figure to align with an illustrative example above}

This semantic graph representation allows us to formulate QA as the search for an optimal \emph{support graph}, a subgraph $G$ of the above augmented graph connecting (the semantic graphs of) $Q$ and $A$ via $P$. The reasoning used to answer the question is captured by a variety of requirements or constraints that $G$ must satisfy,
%\dan{Add a very simple e.g., (need to touch Q and A), and maybe less simple example of a requirement?}
as well as a number of desired properties, encapsulating the ``correct'' reasoning, that makes $G$ preferable over other valid support graphs. For instance, a simple requirement is that $G$ must be connected and it must touch both $Q$ and $A$. Similarly, if $G$ includes a verb from an SRL frame, it is preferable to also include the corresponding subject. Finally, the resulting constrained optimization problem is formulated as an Integer Linear Program (ILP), and optimized using an off-the-shelf ILP solver.

This formalism may be viewed as a generalization of systems that reason over tables of knowledge~\cite{cohen2000:joins,tableilp2016:ijcai}: instead of operating over table rows (which are akin to labeled sequence graphs or predicate-argument graphs), we operate over a much richer class of semantic graphs. It can also be viewed as a generalization of the recent \tupleinf\ system~\cite{khot2017tupleinf}, which converts $P$ into a particular kind of semantic abstraction, namely Open IE tuples~\cite{Banko2007OpenIE}.

This generalization to multiple semantic abstractions poses two key technical challenges: (a) unlike clean knowledge-bases (e.g., \namecite{dong2015question}) used in many QA systems, abstractions generated from NLP tools (e.g., SRL) are noisy; and (b) even if perfect, using their output for QA requires delineating what information in $Q$, $A$, and $P$ is relevant for a given question, and what constitutes valid reasoning. The latter is especially challenging when combining information from diverse abstractions that, even though grounded in the same raw text, may not perfectly align. We address these challenges via our ILP formulation, by using our linguistic knowledge about the abstractions to design requirements and preferences for linking these abstractions.

We present a new QA system, \textilp,\footnote{Code available at: {https://github.com/allenai/semanticilp}} based on these ideas, and evaluate it on multiple-choice questions from two domains involving rich linguistic structure and reasoning: elementary and middle-school level science exams, and early-college level biology reading comprehension. Their data sparsity, as we show, limits the performance of state-of-the-art neural methods such as BiDAF~\cite{seo2016bidirectional}. \textilp, on the other hand, is able to successfully capitalize on existing general-purpose NLP tools in order to outperform existing baselines by 2\%-6\% on the science exams, leading to a new state of the art. It also generalizes well, as demonstrated by its strong performance on biology questions in the \processBank\ dataset~\cite{berant2014modeling}. Notably, while the best existing system for the latter relies on domain-specific structural annotation and question processing, \textilp\ needs neither.




==> intro-old.tex <==
\section{Introduction (OLD)}
\label{sec:intro-old}

\ashish{The intro has a bunch of good text, but I save it for a later section and would instead spin the work quite differently:
\begin{itemize}
    \item Don't spend the whole first (and important!) paragraph on IR and PMI methods.
    
    \item Make (a) the high-level picture and (b) the scope of what we are proposing much more concrete: what kind of QA problems does the work apply to, what is our working hypothesis, and roughly how we propose to solve it? Simple statements about each.
    
    \item The message in the first couple paragraphs could instead be: (a) QA in many domains requires reasoning that goes beyond simple word overlap (in a traditional sense or in a distributional space, possibly via neural methods) or statistical association. (b) Most QA systems that perform such reasoning assume access to a knowledge base in a particular representation formalism (give examples). (c) These systems are, therefore, limited by the knowledge available in a certain formalism. (d) Instead, we work under an IR-style hypothesis that the knowledge needed to answer a question is present somewhere in \emph{raw text}, and that one can arrive at the correct answer by \emph{reasoning over semantic abstractions over the text}.
    
    \item How: Given a question (multiple choice?) start with raw text (either in a reading comprehension setting or with IR-retrieved sentences relevant for a given question --- which, BTW, is another reason to not put IR down too much; we rely on it as the starting point!), then annotate with general-purpose NLP tools such as coref resolution, SRL systems, etc. (this needs to be brought out earlier, rather than at the end of Related Work), then view these layers of abstractions as \emph{semantic graphs}, then formulate QA as a search for the optimal subgraph satisfying certain properties, then implement this search as an ILP.
    
    \item End intro with a quantitative preview of the results --- datasets, achievements.
\end{itemize}
}

Question Answering (QA) has been studied for many years and yet one of the fundamental AI challenge. Most systems for this task are based on relatively shallow Information Retrieval (IR) which work under the assumption that answers to many questions of interest are often explicitly stated somewhere~\cite{Kwok2001ScalingQA}, and all one needs, in principle, is access to a sufficiently large corpus. In a similar line statistical correlation techniques (such as those using Pointwise Mutual Information or PMI~\cite{church1989}) operating on large unstructured corpora, work under the assumption that many questions can be answered by looking for words that tend to co-occur with the question words in a large corpus. 


%Knowledge Representation (KR) is a defining step element in design of AI systems.
More recently more sophisticated statistical approaches and structured reasoning (e.g. \cite{seo2016bidirectional,khot2017tupleinf}) have gotten some attention. One of the reasons that there is wide variety of QA solvers is the different assumptions made on Knowledge Representation (KR) in these solvers.  For IR-based and correlations-based solvers, the key representation is the \textit{raw}-text, or statistics directly (online or offline) extracted from it. Tables of knowledge resulted in \tableilp\cite{cohen2000:joins,tableilp2016:ijcai}, tuple-based knowledge resulted in \tupleinf \cite{khot2017tupleinf}, knowledge-graphs inspired plethora of work (e.g. see \cite{dong2015question}). While having structure in the input knowledge makes it easy to make assumptions about the expected form of the knowledge, it is not clear whether the existing representations are sufficient for sustainable progress in QA systems. 

% on tableilp: 
% semi-structured knowledge represented in the form of $n$-ary predicates over natural language text \addedA{\cite{aristo2016:combining}}. For example, a simple country-hemisphere table represents the binary predicate $r_{\text{ctry-hems}}(c,h)$ with instances such as (Australia, Southern) and (Canada, Northern). Since table content is specified in natural language, the same entity is often represented differently in different tables, posing an additional inference challenge.

In this work we propose a system a structured system, which uses \textit{raw} text as the input knowledge, alongside its general-purpose annotations. 
Our propose system, \textilp\ uses raw text as the core representations, decorated with layers of general-purpose NLP annotations. The knowledge of each annotation layer, the \textit{abstract graph} belongs to certain class of graphs which characterizes its properties. 
%(hence named ``semi-structured"). 
This is rather in contrast with the commonly-pursued approach for structured QA systems which expect the input knowledge to be in one clean form or another (e.g. an RDF graph, a table, semantic parse, etc). 
Our abstraction of knowledge is used for all the inputs to the system, i.e. a question, a bunch of answer-options, and a paragraph that potentially supports one of the answers. Question answering is modelled as finding a support subgraph on a bigger graph which we will construction on top of the knowledge representation.  More concretely, we formulate the problem as 
% Our system is formulated as 
an Integer Linear Program (ILP), which creates an optimization problem by combining representation of question, its answer-option and a knowledge paragraph. By leveraging different views, we propose a few interesting reasoning patterns on top of which we simulate chaining multiple pieces of information and combining parallel evidence. 

% explain the reasoning 
One key premise in our design is robustness to different forms of expressing an idea or an event. Our reasoning formulation, as we will delineate later, implicitly models various textual variations of text, and in fact, sub-graph optimization can be thought of as a search in space of textual paraphrases. Consider the following snippet:
\begin{framed}
\footnotesize \emph { 
A few weeks ago, \textbf{Chelsea purchased Alvaro Morata}. The Spaniard looked like he was set for a move to Old Trafford for the majority of the summer only for Manchester United to sign Romelu Lukaku instead, paving the way for Morata to finally move to Chelsea for an initial \pounds 56m. ...   
%The 24-year-old is in line to make his full Chelsea debut on Sunday against Tottenham at Wembley on Sunday having come off the bench in the season’s curtain raiser against Burnley last weekend.   
%He made a positive start to life in west London with a goal and an assist despite that defeat and Conte insisted that given today market – where Liverpool are rejecting £110m+ offers for Philippe Coutinho – Morata is a bargain signing for the Blues. After signing Morata, Conte spoke publically of how Spurs striker Kane would have been is ideal signing but he tried to clarify those comments by insisting Morata can have a similar impact to the Englishman. 
}
\end{framed}
And consider the following question: 
\begin{framed}
\small  
\noindent
\emph { Who did Chelsea purchase?  \\ 
\checkmark (A)  Alvaro Morata  \;   (B) Old Trafford  \; (C) Romelu Lukaku %  \;  (D) Manchester United 
}
\end{framed}
Given the bold-faced sub-phrase in the snippet, answering this question is relatively easy via simple word-matching. However, the bold-faced sentence could have been worded in many different ways. Imagine the bold-faced text in the snippet is replaced the following: \emph{``Chelsea is hoping to have a great start this season by actively hunting for new players in the transfer period. Morata, the recent acquisition by the team, will start for the team tomorrow."}. Now answering the text is much trickier than before. Our reasoning for this example paragraph is depicted in Figure~\ref{fig:morata-visualization}, where the knowledge representation of different components and the reasoning alignment is depicted (details in later sections).
% \begin{framed}
% \footnotesize
    % \emph{ 
    % \begin{itemize}
        % \item Chelsea acquired Alvaro Morata.  
        % \item Real Madrid sold Alvaro Morata to Chelsea. 
        % \item Alvaro Morata's recent acquisition by Chelsea have given extra hope for it fans.  
        % \item Chelsea broke its previous records by purchasing Morata from Real Madrid.
        % \item Morata hinted at his purchase. Later that day Chelsea announced the purchase.  
        % \item Recent purchase for Chelsea, Alvaro Morata will start for Chelsea tomorrow.  
    % \end{itemize}
    % }
% \end{framed}

\begin{figure}% [ht]
    \centering
    % \begin{framed}
    \includegraphics[trim=-0.00cm 3.7cm 0cm -0.00cm, scale=0.53]{figures/Chelseaishopingtohaveagreatstartthisseason3}
    % \end{framed}
    \caption{Depiction of \textilp\ reasoning for the example paragraph given in the paragraph. 
    The knowledge representation of question, answers, knowledge snippet are shown in a colored boxes (blue, green, yellow, respectively). The red nodes and edges are the aligned (used) elements. In reality there are many many other annotations associated with each text that are unaligned (hence not shown). 
    }
    \label{fig:morata-visualization}
\end{figure}

\daniel{Final paragraph, say something on results. }

% This suggests that a combination of a rich and fine-grained constraint language, namely ILP,
% even with a publicly available solver
% is more effective in practice than various MLN formulations of the task. Further, while the scalability of the MLN formulations 
%  was limited to very few (typically one or two) selected science rules at a time, our approach easily scales to hundreds of relevant scientific facts.
% It also complements the kind of questions amenable to IR and PMI techniques, as is evidenced by the fact that a combination (trained using simple Logistic Regression \addedA{\cite{aristo2016:combining}}) of \tableilp\ with IR and PMI results in a significant (+10\% absolute) boost in the score compared to IR alone.

% Our ablation study suggests that
% combining facts from multiple tables or multiple rows within a table plays an important role in \tableilp's performance. 
% We also show that \tableilp\ benefits from the table structure, by comparing it with an IR system using the same knowledge (the table rows) but expressed as simple sentences; \tableilp\ scores significantly (+10\%) higher. Finally, we demonstrate that our approach is robust to a simple perturbation of incorrect answer options: while the simple perturbation results in a relative drop of 20\% and 33\% in the performance of IR and PMI methods, respectively, it affects \tableilp's performance by only 12\%.


==> ncfyfxrcnwktzvckdjwgzbbmhdqtycrt copy/intro-no-longer-used.tex <==

\section{Introduction}

Question answering (QA) is a fundamental challenge in AI, particularly in natural language processing (NLP) and reasoning. We consider the multiple-choice setting where $Q$ is a question, $A$ is a set of answer candidates, and the knowledge required for answering $Q$ is available in the form of raw text $P$. This setting applies naturally to reading comprehension questions, as well as to open format multiple-choice questions for which information retrieval (IR) techniques are able to obtain relevant text from a corpus.

Several state-of-the-art QA systems excel at locating the correct answer in $P$ based on proximity to question words, the distributional semantics of the text, answer type, etc \cite{aristo2016:combining},
% \daniel{cite something here?}. Even the best solvers
however, often struggle with questions that require some form of reasoning or appeal to a more subtle 
%linguistic 
understanding of the supporting text or the question. We demonstrate that we can use existing NLP modules, such as semantic role labeling (SRL) systems with respect to multiple predicate types (verbs, prepositions, nominals, etc.),
%\daniel{predicates $\rightarrow$ predicate types}, 
%\dan{Note that most people think of SRL only wrt verbs; thus the change.}
to derive multiple semantic views of the text and perform reasoning over these views to answer a variety of questions.

% {\color{blue}
As an example, consider the following snippet of sports news text and an associated question:
\begin{framed}
%\vspace{-1.5ex}
\noindent\footnotesize\emph{\noindent$P$: Teams are under pressure after PSG purchased Neymar this season. \textbf{Chelsea purchased Morata}. The Spaniard looked like he was set for a move to Old Trafford for the majority of the summer only for Manchester United to sign Romelu Lukaku instead, paving the way for Morata to finally move to Chelsea for an initial \pounds 56m.
%The 24-year-old is in line to make his full Chelsea debut on Sunday against Tottenham at Wembley on Sunday having come off the bench in the season’s curtain raiser against Burnley last weekend.   
%He made a positive start to life in west London with a goal and an assist despite that defeat and Conte insisted that given today market – where Liverpool are rejecting £110m+ offers for Philippe Coutinho – Morata is a bargain signing for the Blues. After signing Morata, Conte spoke publically of how Spurs striker Kane would have been is ideal signing but he tried to clarify those comments by insisting Morata can have a similar impact to the Englishman. 
% }
% \end{framed}
% And consider the following question: 
% \begin{framed}
% \small
\\
\noindent
$Q$: Who did Chelsea purchase this season?  \\ 
$A$: \{\checkmark Alvaro Morata, Neymar, Romelu Lukaku \}%  \;  (D) Manchester United
}
%\vspace{-1.5ex}
\end{framed}

Given the bold-faced text $P'$ in $P$, simple word-matching suffices to correctly answer $Q$. However, $P'$ could have stated the same information in many different ways. As paraphrases become more complex, they begin to involve more linguistic constructs such as coreference, punctuation, prepositions, and nominals. This makes understanding the text, and thus the QA task, more challenging.

For instead, $P'$ could instead say \emph{Morata is the recent \textbf{acquisition} by Chelsea}. This simple looking transformation can be surprisingly confusing for highly successful systems such as \bidaf~\cite{seo2016bidirectional}, which produces the partially correct phrase \emph{``Neymar this season.\ Morata''}. On the other hand, one can still answer the question confidently by abstracting relevant parts of $Q$ and $P$, and connecting them appropriately. Specifically, a verb SRL frame for $Q$ would indicate that we seek the object of the verb \emph{purchase}, a nominal SRL frame for $P'$ would capture that the \emph{acquisition} was of Morata and was done by Chelsea, and textual similarity would align \emph{purchase} with \emph{acquisition}.

\begin{figure}[ht]
    \centering
    % \begin{framed}
    % \includegraphics[trim=-0.00cm 3.7cm 0cm -0.00cm, scale=0.53]{figures/Chelseaishopingtohaveagreatstartthisseason3}
    % \end{framed}
    % \includegraphics[trim=-0.00cm 2.5cm 2.5cm -0.00cm, scale=0.55]{figures/cropped_morata-simplfied-cropped.pdf}
    \includegraphics[trim=-0.00cm 0cm 0cm -0.00cm, scale=0.55]{figures/cropped_morata-simplfied-cropped.pdf}
    \caption{Depiction of \textilp\ reasoning for the example paragraph given in the text.
    Semantic abstractions of the question, answers, knowledge snippet are shown in different colored boxes (blue, green, and yellow, resp.). Red nodes and edges are the elements that are aligned (used) for supporting the correct answer. There are many other unaligned (unused) annotations associated with each piece of text that are omitted for clarity. 
    }
    \label{fig:morata-visualization}
\end{figure}

Similarly, suppose $P'$ instead said \emph{Morata\textbf{,} the recent acquisition \textbf{by} Chelsea\textbf{,} will start for the team tomorrow.} \bidaf\ now incorrectly chooses Neymar as the answer, presumably due to its proximity to the words \emph{purchased} and \emph{this season}. However, with the right abstractions, one could still arrive at the correct answer as depicted in Figure~\ref{fig:morata-visualization} for our proposed system, \textilp. This reasoning uses comma SRL to realize that the Morata is referring to the \emph{acquisition}, and a preposition SRL frame to capture that the acquisition was done \emph{by} Chelsea.

One can continue to make $P'$ more complex. For example, $P'$ could introduce the need for coreference resolution by phrasing the information as: \emph{\textbf{Chelsea} is hoping to have a great start this season by actively hunting for new players in the transfer period. Morata, the recent acquisition by the team, will start for \textbf{the team} tomorrow.} Nevertheless, with appropriate semantic abstractions of the text, the underlying reasoning remains relatively simple. 

% such as:
% \begin{framed}
% \vspace{-3ex}
% \footnotesize
%     \emph{ 
%     \begin{enumerate}[leftmargin=0.3cm]
%         \item Chelsea acquired Alvaro Morata.  
%         \item Real Madrid sold Alvaro Morata to Chelsea. 
%         % \item Alvaro Morata's recent acquisition by Chelsea has given extra hope for its fans.  
%         \item Chelsea broke its previous record by purchasing Morata from Real Madrid. \ashish{SQuAD: Morata from Real Madrid}
%         \item Morata hinted at his purchase. Later that day Chelsea announced the purchase.  
%         \item Recent purchase for Chelsea, Alvaro Morata, will start for Chelsea tomorrow.
%         \item Chelsea is hoping to have a great start this season by actively hunting for new players in the transfer period. Morata, the recent acquisition by the team, will start for the team tomorrow.
%     \end{enumerate}
%     }
% \vspace{-2ex}
% \end{framed}

% The first paraphrasing of $P'$ relies on synonymy between \emph{purchased} and \emph{acquired}, a gap easily bridged using resources such as WordNet~\cite{miller1995wordnet} or low-dimensional word embeddings~\cite{mikolov2013distributed}. The second requires understanding that \emph{X purchased Y} is the same as \emph{Y was sold to X}, which methods using contextual verb embeddings, such as LSTM based neural models~\cite{?}, may be able to address. \daniel{instead of this I would say, ``The second requires understanding that \emph{X purchased Y} is the same as \emph{Y was sold to X}, which resources like PropBank~\cite{kingsbury2002treebank} would help to answer."} \ashish{Agreed with the explanation, although, especially since even we don't use PropBank and get it right, I would instead change the rephrasing of $T'$ so that it requires more than just soft word distance but a state-of-the-art system like BiDAF \emph{can} get it correct. Then say what it cannot get.}
% \dan{Are you sure that LSTM based  systems get it for the right reason? Or only because it's the only NE option? Can you try to add deceiving entities?}
% \ashish{Not sure about LSTM. The text does have all other answer options (also NEs) mentioned in the second sentence of the paragraph.}
% \dan{Maybe it's sufficient to say: "requires understanding that \emph{X purchased Y} is the same as \emph{Y was sold to X}"; [or add also] a lexico-structural pattern that can be learned from a large QA collection only for the most common lexical items.}
% \ashish{I like the fancy last sentence, in part because it yields that existing systems \emph{can} do this, at least for common terms.}
% % side note: Propbank indeed helps us answer this. If you go to the "sell" frame, it labels subject as "buyer": https://github.com/propbank/propbank-frames/blob/master/frames/sell.xml#L21
% % }


Given sufficiently large QA training data, one could conceivably perform end-to-end training (e.g., using a deep learning method) to address these linguistic challenges. However, existing large scale QA datasets such as SQuAD~\cite{Rajpurkar2016SQuAD10} often either have a limited linguistic richness or do not necessarily need reasoning to arrive at the answer~\cite{Jia2017AdversarialEF}. 
% \ashish{update citation to point to EMNLP (I think)} 
%\danchange{
Consequently, the resulting models do not transfer easily to other domains.
%}
%\dan{is there a reference to cite here?; can we give the performance of a good Squad system on Aristo?} \ashish{added SQuAD-trained BiDAF performance on Aristo. Helpful or risky claim?}. 
For instance, the above mentioned BiDAF model trained on the SQuAD dataset performs substantially worse than a simple IR approach on our datasets. On the other hand, many of the QA collections in domains that require some form of reasoning, such as the science questions we use, are small  
%, suffer from the issue of \emph{data sparsity}. Their small size 
(100s to 1000s of questions). This brings into question the viability of the aforementioned paradigm that attempts 
%makes it difficult, if not impossible, 
to learn everything from only the QA training data. %One is thus limited to fine tuning parameters of a system pre-trained on a different, larger dataset.
% \dan{rephrased the previous paragraph a bit; please check}\ashish{nice!}

Towards the goal of effective structured reasoning in the presence of data sparsity, we propose to use a rich set of general-purpose, pre-trained NLP tools to create various \emph{semantic abstractions} of the raw text\footnote{This applies to all three inputs of the system: $Q$, $A$, and $P$.} in a domain independent fashion, as illustrated for an example in Figure~\ref{fig:morata-visualization}.
%
%For instance, \ashish{TO-DO: connect back to the illustrative examples above}
% {\color{blue}
% in the 3rd rephrasing above, a semantic role labeling (SRL) system for verbs may identify \emph{Chelsea} as the \emph{purchaser}, despite the presence of several other words in between the verb and its subject. In the 4th rephrasing, a coreference system may reveal that the two mentions of \emph{purchase} refer to the same real-life event. An SRL system for the semantics of commas may similarly identify, in the 5th rephrasing, \emph{Alvaro Morata} as being interchangeable with \emph{recent purchase}. Finally, as the last rephrasing illustrates, one may need to resort to \emph{multiple semantic abstractions} simultaneously.
% }
%
We represent these semantic abstractions as \emph{families of graphs}, where the family (e.g., trees, clusters, labeled predicate-argument graphs, etc.) is chosen to match the nature of the abstraction (e.g., parse tree, coreference sets, SRL frames, etc., respectively). The collection of semantic graphs is then augmented with inter- and intra-graph edges capturing lexical similarity (e.g., word-overlap score or word2vec distance).
%Figure~\ref{fig:morata-visualization} illustrates what such a graph looks like. \ashish{TO-DO: change figure to align with an illustrative example above}

This semantic graph representation allows us to formulate QA as the search for an optimal \emph{support graph}, a subgraph $G$ of the above augmented graph connecting (the semantic graphs of) $Q$ and $A$ via $P$. The reasoning used to answer the question is captured by a variety of requirements or constraints that $G$ must satisfy,
%\dan{Add a very simple e.g., (need to touch Q and A), and maybe less simple example of a requirement?}
as well as a number of desired properties, encapsulating the ``correct'' reasoning, that makes $G$ preferable over other valid support graphs. For instance, a simple requirement is that $G$ must be connected and it must touch both $Q$ and $A$. Similarly, if $G$ includes a verb from an SRL frame, it is preferable to also include the corresponding subject. Finally, the resulting constrained optimization problem is formulated as an Integer Linear Program (ILP), and optimized using an off-the-shelf ILP solver.

This formalism may be viewed as a generalization of systems that reason over tables of knowledge~\cite{cohen2000:joins,tableilp2016:ijcai}: instead of operating over table rows (which are akin to labeled sequence graphs or predicate-argument graphs), we operate over a much richer class of semantic graphs. It can also be viewed as a generalization of the recent \tupleinf\ system~\cite{khot2017tupleinf}, which converts $P$ into a particular kind of semantic abstraction, namely Open IE tuples~\cite{Banko2007OpenIE}.

This generalization to multiple semantic abstractions poses two key technical challenges: (a) unlike clean knowledge-bases (e.g., \namecite{dong2015question}) used in many QA systems, abstractions generated from NLP tools (e.g., SRL) are noisy; and (b) even if perfect, using their output for QA requires delineating what information in $Q$, $A$, and $P$ is relevant for a given question, and what constitutes valid reasoning. The latter is especially challenging when combining information from diverse abstractions that, even though grounded in the same raw text, may not perfectly align. We address these challenges via our ILP formulation, by using our linguistic knowledge about the abstractions to design requirements and preferences for linking these abstractions.

We present a new QA system, \textilp,\footnote{Code available at: {https://github.com/allenai/semanticilp}} based on these ideas, and evaluate it on multiple-choice questions from two domains involving rich linguistic structure and reasoning: elementary and middle-school level science exams, and early-college level biology reading comprehension. Their data sparsity, as we show, limits the performance of state-of-the-art neural methods such as BiDAF~\cite{seo2016bidirectional}. \textilp, on the other hand, is able to successfully capitalize on existing general-purpose NLP tools in order to outperform existing baselines by 2\%-6\% on the science exams, leading to a new state of the art. It also generalizes well, as demonstrated by its strong performance on biology questions in the \processBank\ dataset~\cite{berant2014modeling}. Notably, while the best existing system for the latter relies on domain-specific structural annotation and question processing, \textilp\ needs neither.




==> ncfyfxrcnwktzvckdjwgzbbmhdqtycrt copy/intro-old.tex <==
\section{Introduction (OLD)}
\label{sec:intro-old}

\ashish{The intro has a bunch of good text, but I save it for a later section and would instead spin the work quite differently:
\begin{itemize}
    \item Don't spend the whole first (and important!) paragraph on IR and PMI methods.
    
    \item Make (a) the high-level picture and (b) the scope of what we are proposing much more concrete: what kind of QA problems does the work apply to, what is our working hypothesis, and roughly how we propose to solve it? Simple statements about each.
    
    \item The message in the first couple paragraphs could instead be: (a) QA in many domains requires reasoning that goes beyond simple word overlap (in a traditional sense or in a distributional space, possibly via neural methods) or statistical association. (b) Most QA systems that perform such reasoning assume access to a knowledge base in a particular representation formalism (give examples). (c) These systems are, therefore, limited by the knowledge available in a certain formalism. (d) Instead, we work under an IR-style hypothesis that the knowledge needed to answer a question is present somewhere in \emph{raw text}, and that one can arrive at the correct answer by \emph{reasoning over semantic abstractions over the text}.
    
    \item How: Given a question (multiple choice?) start with raw text (either in a reading comprehension setting or with IR-retrieved sentences relevant for a given question --- which, BTW, is another reason to not put IR down too much; we rely on it as the starting point!), then annotate with general-purpose NLP tools such as coref resolution, SRL systems, etc. (this needs to be brought out earlier, rather than at the end of Related Work), then view these layers of abstractions as \emph{semantic graphs}, then formulate QA as a search for the optimal subgraph satisfying certain properties, then implement this search as an ILP.
    
    \item End intro with a quantitative preview of the results --- datasets, achievements.
\end{itemize}
}

Question Answering (QA) has been studied for many years and yet one of the fundamental AI challenge. Most systems for this task are based on relatively shallow Information Retrieval (IR) which work under the assumption that answers to many questions of interest are often explicitly stated somewhere~\cite{Kwok2001ScalingQA}, and all one needs, in principle, is access to a sufficiently large corpus. In a similar line statistical correlation techniques (such as those using Pointwise Mutual Information or PMI~\cite{church1989}) operating on large unstructured corpora, work under the assumption that many questions can be answered by looking for words that tend to co-occur with the question words in a large corpus. 


%Knowledge Representation (KR) is a defining step element in design of AI systems.
More recently more sophisticated statistical approaches and structured reasoning (e.g. \cite{seo2016bidirectional,khot2017tupleinf}) have gotten some attention. One of the reasons that there is wide variety of QA solvers is the different assumptions made on Knowledge Representation (KR) in these solvers.  For IR-based and correlations-based solvers, the key representation is the \textit{raw}-text, or statistics directly (online or offline) extracted from it. Tables of knowledge resulted in \tableilp\cite{cohen2000:joins,tableilp2016:ijcai}, tuple-based knowledge resulted in \tupleinf \cite{khot2017tupleinf}, knowledge-graphs inspired plethora of work (e.g. see \cite{dong2015question}). While having structure in the input knowledge makes it easy to make assumptions about the expected form of the knowledge, it is not clear whether the existing representations are sufficient for sustainable progress in QA systems. 

% on tableilp: 
% semi-structured knowledge represented in the form of $n$-ary predicates over natural language text \addedA{\cite{aristo2016:combining}}. For example, a simple country-hemisphere table represents the binary predicate $r_{\text{ctry-hems}}(c,h)$ with instances such as (Australia, Southern) and (Canada, Northern). Since table content is specified in natural language, the same entity is often represented differently in different tables, posing an additional inference challenge.

In this work we propose a system a structured system, which uses \textit{raw} text as the input knowledge, alongside its general-purpose annotations. 
Our propose system, \textilp\ uses raw text as the core representations, decorated with layers of general-purpose NLP annotations. The knowledge of each annotation layer, the \textit{abstract graph} belongs to certain class of graphs which characterizes its properties. 
%(hence named ``semi-structured"). 
This is rather in contrast with the commonly-pursued approach for structured QA systems which expect the input knowledge to be in one clean form or another (e.g. an RDF graph, a table, semantic parse, etc). 
Our abstraction of knowledge is used for all the inputs to the system, i.e. a question, a bunch of answer-options, and a paragraph that potentially supports one of the answers. Question answering is modelled as finding a support subgraph on a bigger graph which we will construction on top of the knowledge representation.  More concretely, we formulate the problem as 
% Our system is formulated as 
an Integer Linear Program (ILP), which creates an optimization problem by combining representation of question, its answer-option and a knowledge paragraph. By leveraging different views, we propose a few interesting reasoning patterns on top of which we simulate chaining multiple pieces of information and combining parallel evidence. 

% explain the reasoning 
One key premise in our design is robustness to different forms of expressing an idea or an event. Our reasoning formulation, as we will delineate later, implicitly models various textual variations of text, and in fact, sub-graph optimization can be thought of as a search in space of textual paraphrases. Consider the following snippet:
\begin{framed}
\footnotesize \emph { 
A few weeks ago, \textbf{Chelsea purchased Alvaro Morata}. The Spaniard looked like he was set for a move to Old Trafford for the majority of the summer only for Manchester United to sign Romelu Lukaku instead, paving the way for Morata to finally move to Chelsea for an initial \pounds 56m. ...   
%The 24-year-old is in line to make his full Chelsea debut on Sunday against Tottenham at Wembley on Sunday having come off the bench in the season’s curtain raiser against Burnley last weekend.   
%He made a positive start to life in west London with a goal and an assist despite that defeat and Conte insisted that given today market – where Liverpool are rejecting £110m+ offers for Philippe Coutinho – Morata is a bargain signing for the Blues. After signing Morata, Conte spoke publically of how Spurs striker Kane would have been is ideal signing but he tried to clarify those comments by insisting Morata can have a similar impact to the Englishman. 
}
\end{framed}
And consider the following question: 
\begin{framed}
\small  
\noindent
\emph { Who did Chelsea purchase?  \\ 
\checkmark (A)  Alvaro Morata  \;   (B) Old Trafford  \; (C) Romelu Lukaku %  \;  (D) Manchester United 
}
\end{framed}
Given the bold-faced sub-phrase in the snippet, answering this question is relatively easy via simple word-matching. However, the bold-faced sentence could have been worded in many different ways. Imagine the bold-faced text in the snippet is replaced the following: \emph{``Chelsea is hoping to have a great start this season by actively hunting for new players in the transfer period. Morata, the recent acquisition by the team, will start for the team tomorrow."}. Now answering the text is much trickier than before. Our reasoning for this example paragraph is depicted in Figure~\ref{fig:morata-visualization}, where the knowledge representation of different components and the reasoning alignment is depicted (details in later sections).
% \begin{framed}
% \footnotesize
    % \emph{ 
    % \begin{itemize}
        % \item Chelsea acquired Alvaro Morata.  
        % \item Real Madrid sold Alvaro Morata to Chelsea. 
        % \item Alvaro Morata's recent acquisition by Chelsea have given extra hope for it fans.  
        % \item Chelsea broke its previous records by purchasing Morata from Real Madrid.
        % \item Morata hinted at his purchase. Later that day Chelsea announced the purchase.  
        % \item Recent purchase for Chelsea, Alvaro Morata will start for Chelsea tomorrow.  
    % \end{itemize}
    % }
% \end{framed}

\begin{figure}% [ht]
    \centering
    % \begin{framed}
    \includegraphics[trim=-0.00cm 3.7cm 0cm -0.00cm, scale=0.53]{figures/Chelseaishopingtohaveagreatstartthisseason3}
    % \end{framed}
    \caption{Depiction of \textilp\ reasoning for the example paragraph given in the paragraph. 
    The knowledge representation of question, answers, knowledge snippet are shown in a colored boxes (blue, green, yellow, respectively). The red nodes and edges are the aligned (used) elements. In reality there are many many other annotations associated with each text that are unaligned (hence not shown). 
    }
    \label{fig:morata-visualization}
\end{figure}

\daniel{Final paragraph, say something on results. }

% This suggests that a combination of a rich and fine-grained constraint language, namely ILP,
% even with a publicly available solver
% is more effective in practice than various MLN formulations of the task. Further, while the scalability of the MLN formulations 
%  was limited to very few (typically one or two) selected science rules at a time, our approach easily scales to hundreds of relevant scientific facts.
% It also complements the kind of questions amenable to IR and PMI techniques, as is evidenced by the fact that a combination (trained using simple Logistic Regression \addedA{\cite{aristo2016:combining}}) of \tableilp\ with IR and PMI results in a significant (+10\% absolute) boost in the score compared to IR alone.

% Our ablation study suggests that
% combining facts from multiple tables or multiple rows within a table plays an important role in \tableilp's performance. 
% We also show that \tableilp\ benefits from the table structure, by comparing it with an IR system using the same knowledge (the table rows) but expressed as simple sentences; \tableilp\ scores significantly (+10\%) higher. Finally, we demonstrate that our approach is robust to a simple perturbation of incorrect answer options: while the simple perturbation results in a relative drop of 20\% and 33\% in the performance of IR and PMI methods, respectively, it affects \tableilp's performance by only 12\%.

